When Anomaly Mediation is UV Sensitive

Despite its successes---such as solving the supersymmetric flavor problem---anomaly mediated supersymmetry breaking is untenable because of its prediction of tachyonic sleptons. An appealing solution to this problem was proposed by Pomarol and Rattazzi where a threshold controlled by a light field deflects the anomaly mediated supersymmetry breaking trajectory, thus evading tachyonic sleptons. In this paper we examine an alternate class of deflection models where the non-supersymmetric threshold is accompanied by a heavy, instead of light, singlet. The low energy form of this model is the so-called extended anomaly mediation proposed by Nelson and Weiner, but with potential for a much higher deflection threshold. The existence of this high deflection threshold implies that the space of anomaly mediated supersymmetry breaking deflecting models is larger than previously thought.

==> cmds/preamble-cmd-spectrum_draw.tex <==
\let\gobbleEnd=\relax
\newcommand{\drawmasslines}[2]{\gobblemasslist#2,\gobbleHalt\gobbleEnd}
\newcommand{\gobbleHalt}{\@\@\@\@}

\def\gobblemasslist(#1,#2,[#3,#4]),#5\gobbleEnd{%
\ifthenelse{ \equal{#5}{\gobbleHalt} }%
	{%
	\put(\xCoord,#2){\line(1,0){\masslinelen} \raisebox{#4}{\hspace{#3}$#1$}}%
	}%
% Else
	{%
	\put(\xCoord,#2){\line(1,0){\masslinelen} \raisebox{#4}{\hspace{#3}$#1$}}%
	\gobblemasslist#5\gobbleEnd%
	}%
}%


\newlength{\oldunitlength}
\setlength{\oldunitlength}{\the\unitlength}
\newcommand{\masslinelen}{50}
\newcommand{\xCoordColOne}{10}
\newcommand{\xCoordColTwo}{120}
\newcommand{\xCoordColThree}{230}
\newcommand{\xCoordColFour}{340}
\newcommand{\xCoordColFive}{450}
\newcommand{\xCoord}{}
\newcommand{\defaultX}{1mm}
\newcommand{\defaultY}{-0.6ex}
\newcommand{\placetoleft}{-1.4cm}
\newcommand{\placetoleftnudgeright}{-1.33cm}
\newcommand{\placetoleftnudgeleft}{-1.47cm}
\newcommand{\slightlyraised}{-0.4ex}
\newcommand{\slightlylowered}{-0.8ex}


